AutoHallusion: Automatic Generation of Hallucination Benchmarks for Vision-Language Models

Large vision-language models (LVLMs) are prone to hallucinations, where certain contextual cues in an image can trigger the language module to produce overconfident and incorrect reasoning about abnormal or hypothetical objects. While some benchmarks have been developed to investigate LVLM hallucinations, they often rely on hand-crafted corner cases whose failure patterns may not generalize well. Additionally, fine-tuning on these examples could undermine their validity. To address this, we aim to scale up the number of cases through an automated approach, reducing human bias in crafting such corner cases. This motivates the development of AutoHallusion, the first automated benchmark generation approach that employs several key strategies to create a diverse range of hallucination examples. Our generated visual-question pairs pose significant challenges to LVLMs, requiring them to overcome contextual biases and distractions to arrive at correct answers. AutoHallusion enables us to create new benchmarks at the minimum cost and thus overcomes the fragility of hand-crafted benchmarks. It also reveals common failure patterns and reasons, providing key insights to detect, avoid, or control hallucinations. Comprehensive evaluations of top-tier LVLMs, e.g., GPT-4V(ision), Gemini Pro Vision, Claude 3, and LLaVA-1.5, show a 97.7% and 98.7% success rate of hallucination induction on synthetic and real-world datasets of AutoHallusion, paving the way for a long battle against hallucinations. The codebase and data can be accessed at https://github.com/wuxiyang1996/AutoHallusion.

==> section/1-intro-back.tex <==
\section{Introduction}

\wxy{This is the merged version of all comments before 06/03}

The mystery of how humans form their memory by interpreting and understanding the world around them is a long-lasting research topic in cognitive science \cite{bartlett1995remembering, brewer1981role, trevarthen1977cognition}. Psychologists use schema, a knowledge structure that organizes categories of information and the relationships among them, to interpret the formulation process of human memory \cite{dimaggio1997culture, boutyline2021cultural, rumelhart2017schemata}. People use schemata to interpret and memorize training data they encounter and learn new schemata through accretion, tuning, and reconstruction \cite{rumelhart1976accretion}.

The formulation of associative memory \cite{anderson2014human} connects various schemata from training data and performs associative priming when encountering related concepts \cite{de2019auditory}. For example, the schemata \textit{computer monitor} and \textit{keyboard} form an associative memory due to their high likelihood of co-occurrence in the real world. Once a \textit{computer monitor} presents in a scene, this schema serves as a priming that reminds humans to think about the schema \textit{keyboard}. 

However, such associative memory among schemata leaves the space for hallucinations \cite{el2010hallucinations, chiu1989differential}. Hallucinations may occur when irregular schemata perturb the expected combination of schemata, leading to cognitive dissonance due to conflicts in interpretation for schemata \cite{aronson1969theory, harmon2019introduction}, or intentionally removing some essential schemata from the combination of schemata that leads to the expectancy violation due to such absence \cite{burgoon1993interpersonal, burgoon1988nonverbal}. In such cases, the human brain may misinterpret or distort the actual perception due to the prior memory associated with the priming from the existing schemata.

Back to the \textit{computer monitor} and \textit{keyboard} example, instead of placing a \textit{keyboard} on the front of \textit{computer monitor}, we place an \textit{irregular schema}, like \textit{octopus}, and probe the existence of the object on the front of \textit{computer monitor}, the hallucination answer of this question is to insist the existence of \textit{keyboard} that comes from the memory, not \textit{octopus} from the actual perception, which is a case of \textit{cognitive dissonance}. On the other hand, we provide two related schemata like the \textit{computer monitor} and \textit{mouse}, while the \textit{keyboard} is still absent. When probing the existence of the object on the front of \textit{computer monitor} and the human provides the wrong answer due to hallucination, this is a case for \textit{expectancy violation} as it cases from the priming of the existing schemata.

Large vision-language models (LVLMs) reveal impressive image-context reasoning abilities, which come from the vast knowledge encoded in their parameters. Given the fact that the training procedure of LVLMs follows a similar pipeline (\textit{i.e.} accretion, tuning, and reconstruction) as humans form their memory, and LVLMs enhance the connection among conceptions through transformer \cite{vaswani2017attention}, they also show their vulnerability to hallucinations when models over-rely on language priors instead of visual context \cite{li2023evaluating, guan2024hallusionbench}, whereas the contextual cues in the input of LVLMs serve as the priming for their language priors.
Previous work \dianqi{citations} has explored creating hallucination cases by adding adversarial objects \cite{rohrbach2018object, li2023evaluating, zhou2023analyzing} or textual information \cite{qraitem2024vision, qian2024easy} or removing relevant information \dianqi{citations}. However, there is no prior work focusing on the automatic generation of hallucination cases, which stems from the rigorous analysis and problem formulation for the emergence of hallucination in LVLMs both from cognitive science and mathematical perspective, which lay the foundation of the main contribution in our work.

\wxy{Need to use terms from cognitive science here, To-Do}

\textbf{Main contributions: } Aware of the role of contextual cues in image-context reasoning tasks of large vision-language models (LVLMs), our work proposes \ours{}, an automated approach to synthesize hallucinative images by exploiting these contextual priors. We present two primary strategies for crafting hallucination cases: inserting abnormal objects negatively correlated with the existing information in the images and erasing hypothetical objects from images rich in contextual information positively correlated with the target objects. We use a series of questions to probe potential hallucination cases in the edited images from two perspectives: the presence of altered contextual elements and the spatial relations between these altered elements and the unaltered elements. 
Hallucinations are highlighted when models provide incorrect answers based on the visual information or deliver inconsistent responses to questions with the same targets in varying contexts. The novelties of our work include:

\begin{itemize*}
    \item We propose an auto-generated approach to synthesize hallucinative images. Our two primary strategies involve inserting abnormal objects that contrast with contextual information and erasing hypothetical objects strongly connected to existing contextual elements. \dianqi{we need to find two simple phrases to represent the two strategies so reviewers can easily remember them through reading the whole paper}    
    % We propose an auto-generated hallucination approach to synthesize visual hallucination cases. We present two primary strategies \dianqi{we need to find two simple phrases to represent the two strategies so reviewers can easily remember them through reading the whole paper} for hallucination creation that either insert abnormal objects versus contextual information or erase hypothetical objects with strong connections with existing contextual elements.
    % \fhc{change to}\fh{We propose an auto-generated approach to synthesize hallucinative images. Our two primary strategies involve inserting abnormal objects that contrast with contextual information or erasing hypothetical objects strongly connected to existing contextual elements.}
    \item We logically analyze the cause \dianqi{what cause? I think we should mention "schema" and "cognition dissonance", so that our proposed methods are well supported by the evidence from cognition field.} of hallucination cases encountered by our approach and propose textual probing methods and corresponding evaluation metrics over the presence and spatial relations of targeting objects with respect to the other contextual elements.  
    \jbgcomment{Agree with Danqi.  I'd go even further and explain what the causes are}
    \item We conduct evaluation experiments on several candidate pipelines following both strategies, along with several baselines and ablation methods over top-tier LVLMs, including GPT-4V(ision), Gemini Pro Vision, Claude 3, and LLaVA1.5. Results show that \ours{} achieves an XX\% attack success rate on the Dall-E generated image cases and a YY\% attack success rate over scene and object images queried from datasets acquired from the real world.
\end{itemize*}

\wxy{Below this is the comments and introduction made before NeurIPS deadline, keep this for reference}

==> section/3-problem_formulation_old.tex <==
\section{Problem Formulation}

In this section, we give some definitions and describe our problem and approach.

\subsection{Definition and Assumptions}

% \noindent\textbf{Definitions:} 

\noindent\textbf{Set Representation of Text Caption:} Let $\mathcal{W}$ be a set of words, descriptions, or relations that are atomic and non-repetitive. For example, it can be a noun, an adjective that is associated with a noun, or the relationship between two objects. Then one accurate caption $T_i$ for image $I$ can be represented as a set $D_i(I)\subset\mathcal{W}$, and the ground truth text representation of an image $I$ can be represented as $Y(I) = \bigcup_{i} D_i(I)$. Let the set representation of the text generated by a VLM regarding the image $I$ be $Pr(y | I)$, and let $\mathcal{I}_{train}$ be the set of training images.


\noindent\textbf{Correctness:} Under the set representation of the text, an response $Pr(y | I)$ is consider correct if $Pr(y | I)\subseteq Y(I)$.

We make the following assumptions:

\noindent\textbf{VLM Hallucination:} Hallucination is inevitable~\cite{xu2024hallucination}. That is, $\exists\ I_h, s.t.\  Pr(y | I_h)\not\subset Y(I_h)$.

\noindent\textbf{VLM Training:} Given a training image set $\mathcal{I}_{train}$, the VLM has the capability to learn the alignment relations of those images to some extent. That is, $\forall I\in \mathcal{I}_{train},\ d(Pr(y | I),\ Y(I)) < \epsilon$, where $d$ measures the distances of the responses and it satisfies that if $d(Pr(y | I),\ Y(I)) < \delta(Pr(y | I))$ for some $\delta$, $Pr(y | I)$ is correct.




\subsection{Goal}

We want to find $I_h\ s.t.\ \exists\ a\in Pr(y | I_h), a\notin Y(I_h)$, so that the hallucination occurs. Essentially, 

\subsection{Approach}

Construct $I_h\ s.t.\ I_h \notin \mathcal{I}_{train}$ and $d(Pr(y | I_h), Y(I_h)) > \delta(Pr(y | I))$ for some $\delta$.



% $max_{T,I} d[ Pr(y | T, I), y(I) ], s.t.  d[ Pr(y | T, I), Pr(y | T) ]  < \epsilon$


% max_{T,I} d[ Pr(y | T, I), y(I) ], s.t.  d[ Pr(y | T, I), Pr(y | T) ]  < \epsilon

% T - input text, I - input image, y - answer/response, y(I) - ground truth, d - distance





==> section/3_-_problem_formulation_-_old_-_06022024.tex <==
\subsection{Definition and Assumptions}
\noindent\textbf{Task Description.} In this work, we are focusing on the hallucination phenomena that exist in the visual question-answering (VQA) task. Specifically, we are interested in those hallucinations emerging from questions regarding the existence and spatial relations among contextual elements, which in most cases are objects, within the given image.

\noindent\textbf{Set Representation of Contextual Elements.} In the image $\mathcal{I}$ provided to the LVLM, many rich but irrelevant contextual information may exist, though we are only interested in those related to the existence and spatial relations of objects. 

Let $\mathcal{I}_{train}$ be the set of training images and $\mathcal{W}$ be the set of binary values, representing all the existence and spatial relations among contextual elements that appeared in $\mathcal{I}_{train}$. For image $\mathcal{I}$, let $\mathcal{W}_I$ be a set of contextual elements in this image, where $\mathcal{W}_I \in \mathcal{W}$ is a subset of all contextual information provided by $I$. Each element in $\mathcal{W}_I$ is a binary element, representing whether the given contextual elements or spatial relations exist in the given image $\mathcal{I}$ \dianqi{keep same style by using $\mathcal{I}$, similarly for $\mathcal{W}$}.
%$0$ means non-existing, and $1$ means existing. 

For example, \wxy{add an illustrative image here} we have an Object $A$ and Object $B$ in the given image $I$, where $A$ is on the left of $B$. In the corresponding set of contextual elements $\mathcal{W}_I$, we have $W_A$ and $W_B$ \dianqi{notation is here confusing, you have two styles: $\mathcal{W}_I$, $\mathcal{W}_A$, but $A$ is within image $I$. a better formulation may be $\mathcal{W}_\mathcal{I} (A, B, C)$ via a function
}, the contextual elements representing the existence of $A$ and $B$, equal to $1$. $W_C$, an contextual element representing the existence of a non-existing element $C$ in $I$, equals to $0$. $W_{A, \{left\}, B}$ is $1$, while $W_{A, \{right\}, B}$ and $W_{A, \{left\}, C}$ are both $0$ as $A$ is on the left, not right, of $B$ and $C$ does not exist\dianqi{refer Visual Genome paper, a better formulation about existence and spatial relation is defining functions \textit{exist(A)} and \textit{on\_the\_left(A, B)}, etc.}.

For a given image $I$, we assume that $\mathcal{W}_I$ is fixed and contains values for all possible contextual elements within $\mathcal{W}$, serving as the ground truth of our further probing for potential hallucinations.

\noindent\textbf{Model Prediction.} In the real world, the LVLMs we use to perform VQA tasks cannot make predictions perfectly matching the ground truth $\mathcal{W}_I$ given image $I$, which inevitably leaves the space for the hallucination~\cite{xu2024hallucination}. The LVLMs may either miss some contextual elements from within the ground truth or even make wrong predictions about certain contextual elements due to hallucinations. 

We take the model predictions for image $I$ as $\mathcal{W}_{I, pred}$. When no hallucinations exist within $\mathcal{W}_{I, pred}$, we take $\mathcal{W}_{I, pred}$ as a subset of $\mathcal{W}_I$. On the other hand, when hallucinations exist within the model predictions for image $I$, we have $\mathcal{W}_{I, pred} \subsetneq \mathcal{W}_I$, which means that the model makes wrong predictions for one or more contextual elements in $\mathcal{W}_{I, pred}$.

\jbgcomment{Prefer $\Pr (y \g I)$ for this so that the kerning and spacing are correct. It is also better if every equation is a noun in a sentence, and not at the start of a sentence.  I think it would also look better to write it as $\mathcal{W}_{I, \mbox{pred}}$}


\noindent\textbf{Objective Function.} The objective function of the LVLM that performs the VQA task given $I$ could be formulated as the procedure of optimizing over the parameters $\theta$ \dianqi{I don't think we optimize $\theta$ ?} of the LVLM to maximize the probability that the model predictions of this LVLM is aligned with the ground truth $\mathcal{W}_I$.
\begin{align}
    \max_{\theta} P(\mathcal{W}_{I, pred} \subsetneq \mathcal{W}_I | I, \theta)
\end{align}
when the LVLM is perfect, \textit{i.e.} $\theta = \theta^*$, when have $P(\mathcal{W}_{I, pred} \subsetneq \mathcal{W}_I | I, \theta) = 1$, \textit{i.e.} this LVLM is always able to make predictions adhere to the ground truth \dianqi{then prob should be 0 instead of 1?}.

\jbgcomment{I'm confused about this step.  Is this over "normal" data or the adversarial data?  In any event, needs a "big" picture explanation of why this is happening.  E.g., we need a fine-tuned model that can\dots }

Split down the probability, $P(\mathcal{W}_{I, pred} \subsetneq \mathcal{W}_I | I, \theta) = 1$ is the product of the probability each element in $\mathcal{W}_{I, pred}$ equals to its ground truth given in $\mathcal{W}_I$, which is 

\begin{align}
    \max_{\theta} \prod_i P(\mathcal{W}^i_{I, pred} = \mathcal{W}^i_I | I, \theta)
\end{align}

Suppose that $\mathcal{W}_{I, pred} = \{A, B\}$ and $\mathcal{W}_{I} = \{A = 0, B = 1, C = 0\}$, then we have \dianqi{super confused by this part, and not sure about what is the purpose of this chain rule}
\begin{align}
    P(\mathcal{W}_{I, pred} \subseteq \mathcal{W}_I | I, \theta)
    =& \prod_i P(\mathcal{W}^i_{I, pred} = \mathcal{W}^i_I | I, \theta) \\
    =& \prod_i P(A = 0 | I, \theta) P(B = 1 | I, \theta) \notag
\end{align}
Since the element $C$ does not exist in the $\mathcal{W}_{I, pred}$ so we do not count the prediction for $C$ into the utlimiate probability for the model prediction. However, for those elements covered by the model predictions, an accurate prediction is necessary otherwise we make hallucinations happen.

\jbgcomment{I'm also confused by this.  It would be good to relate this back to the motivating example.  E.g., X is the image representation, Y is the question about what is on the table, etc.}

\subsection{Hallucination Attacks}
\noindent\textbf{Hallucination Attacks Objective Function.} Given the objective function for the VQA task given $I$, we conduct the objective function for hallucination attacks over the edited image $I'$. The goal of our pipeline is to find the edited image $I'$ with the constrained edition distance $\epsilon$ from the initial image $I$ that minimizes the probability of $\mathcal{W}_{I', pred}$ being a subset of $\mathcal{W}_I'$, \textit{i.e.} the model prediction over image $I'$ is a subset of the ground truth of $I'$.

\jbgcomment{I'd also connect $\mathcal{W}$ back to the example: e.g., find the set that has the lowest probability}

\jbgcomment{What is "edition distance"?   Is that "edit distance"?  EIther way, it is probably good to cite / explain.  Is this in pixel space?}

\jbgcomment{Equation not integrated into a sentence}

\begin{align}
    & \min_{I'} P(\mathcal{W}_{I', pred} \subseteq \mathcal{W}_{I'} | I', \theta) \\
    & s.t. \quad d(I, I') \leq \epsilon \notag
\end{align}

Split down the probability, we have 
\begin{align}
    P(\mathcal{W}_{I', pred} \subseteq \mathcal{W}_{I'} | I', \theta) = \prod_i P(\mathcal{W}^i_{I', pred} = \mathcal{W}^i_{I'} | I', \theta)
\end{align}

which means that once the model fails to make a correct prediction for one or more contextual elements $\mathcal{W}^i_{I'}$, the corresponding probability will drastically drop to $0$, same as the product of probability, \textit{i.e.} $\mathcal{W}_{I', pred} \subsetneq \mathcal{W}_{I'}$, the hallucination over this element happen.

Inspired by this, we propose two major strategies for hallucination attacks. 

\jbgcomment{I think I'd spell these things out a little bit more.  How do you select the new element (e.g., is it a combinatorial search, random and you select the best, etc.)}

\noindent\textbf{Object Insertion Attack.} One way to create a hallucination is to insert an adversary object into the image $I$. The edited ground truth $\mathcal{W}_{I'}$ is given on the basis of $\mathcal{W}_{I}$, leaving all other elements unchanged except setting the existence element of the adversary object as $1$, along with its corresponding spatial relations with respect to other objects within this image. 

\jbgcomment{Again, it would be good to give more detail about how this search happens: randomly delete 1, 2, etc.?  Or find the best.}

\noindent\textbf{Object Erasure Attack.} Another way is to erase an existing object from the image $I$. The edited ground truth $\mathcal{W}_{I'}$ is given on the basis of $\mathcal{W}_{I}$, leaving all other elements unchanged except setting the existence element of the adversary object as $0$, along with its corresponding spatial relations with respect to other objects within this image. 

==> section/3_-_problem_formulation_-_old_-_06042024.tex <==
\section{Problem Formulation}
\wxy{Xiyang: Here I merge several versions and address all comments leave until 06/02, please check}

% \wxy{Think about using T or Q(Query), y_{I} to y_{q, I}, contextual element to C}

\textbf{Definition and Objectives.} We position our objective to find text-image pairs $(Q, I)$ such that the LVLM response is dominant by the prior information of its LLM component only that could be stimulated by the query $Q$ and the guiding text $T$ based on the context within the image $I$, and ignore the ground truth information $Y_{Q, I}$ presented in the image $I$ when queried by the text $Q$. 

% given the image $I$ and the probing text $T$ 

% such that the LVLM response/answer is dominated by its language model (LM) prior $Y_{LM}$, generated when LM is exposed to partial information of $I$ (\textit{i.e.} contextual information about a specific part within the image) in a text form denoted by $T_I$ \dianqi{$T$ represents partial description in image $I$}, but contradicts the ground truth $y_I$ \dianqi{$Y_{I, Q}$} in the given image $I$. \wxy{Check if my understanding to LM is correct}

\textbf{A Case Study.} We have an image $I$ depicting an office. This image $I$ has a coffee maker but no perceivable coffee beans inside. The query $Q$ is the question to probe the existence of the context \textit{coffee beans} this image, which is \textit{''Is there any coffee beans in this image?''}. The ground truth information $Y_{Q, I}$ in this image $I$ when queried by $Q$ is \textit{''There a coffee maker but no coffee beans in this image.''}.
The guiding text $T$ extracted from $I$ is usually a \textbf{partial} fact: \textit{''There is a coffee maker in this image.''} In the hallucination case, the LLM prior $Y_{LLM}$ under this hallucination case might be \textit{''Yes, there are some coffee beans in this image.''} when exposed to the guiding text $T$ and the query $Q$. The LVLM output $Y_{LVLM}$, as it is dominated by its LLM prior $Y_{LLM}$, might produce a similar answer \textit{''Yes, coffee beans could be found in this image.''}. However, $Y_{LVLM}$ contracts to the ground truth information $Y_{Q, I}$, so hallucination happens.

\wxy{I feel that we need an example from the dataset or PS to illustrate this case}

\textbf{Problem Formulation.} For ease of further illustration, we denote the output of LVLM as a function of its input $Q$ and $I$, which is $Y_{LVLM} = f_\mathtt{LVLM}(Q, I)$. Similarly, we use another function to denote the LLM prior as $Y_{LLM} = f_\mathtt{LLM}(Q, T)$. 

To rigorously formulate this problem, we introduce the idea of contextual distance $d$. When two contexts convey similar information or affirm each other, we denote the contextual distance $d$ between the two is small. On the other hand, if two contexts convey rather irrelevant information or contradict each other, we denote the contextual distance $d$ between the two is large.

Hence, we can formulate the high-level objective function given by  Eq.~\ref{equ:high-level} as maximizing the contextual distance between the LVLM output $f_\mathtt{LVLM}(Q, I)$ and the corresponding ground truth information $Y_{Q, I}$, while keeping the contextual distance between $f_\mathtt{LVLM}(Q, I)$ and its LLM prior $f_\mathtt{LLM}(Q, T)$ small enough that the distance between the two is constrained within the upper bound $\epsilon$ denoting the tolerance of the similarity between two contexts. Notably, $T$ could be an empty text when the LLM prior is strong enough to cause hallucination in this case.
\wxy{correct me if my comments on distance is wrong}
\begin{equation}\label{equ:high-level}
    \max_{Q,I} d[f_\mathtt{LVLM}(Q, I), Y_{Q, I}],~~s.t.~~d[f_\mathtt{LLM}(Q, T), f_\mathtt{LVLM}(Q, I)]\leq \epsilon.
\end{equation}

\textbf{Set Representation of Contextual Elements.} Semantically, both query $Q$ and image $I$ provided to the LVLM could be taken as a combination of several contextual elements\footnote{Each contextual element can be a scene, an object, an attribute associated with an object, or the relation between/among multiple objects, similar to the visual genome dataset.}. Using such a set representation of contextual elements, we could reduce the high-level objective function into a more detailed, set-based objective function focusing on the contextual element conveyed by either query $Q$ or image $I$. 

For example, $Q$ can be the query probing the set of contextual elements $\mathcal C_{Q}$ centering about the context $Q$, which could be either in or not in the image $I$. $Y_{Q, I}$ is the ground truth information queried from the image $I$ by the query $Q$ focusing on the contextual elements set $\mathcal C_{Q}$. When the questions $Q$ are all yes/no questions, both the LVLM answer $f_\mathtt{LVLM}(Q, I)$ and the ground truth answer $Y_{Q, I}$ can be parsed to binary strings, \textit{i.e.} $0$ denotes counterfactual answers and $1$ denotes the affirmative answers. Hence, we can use Hamming distance as $d[\cdot,\cdot]$ to compute the contextual distance between two contexts. $T$ can be the indicators (or labels) $\mathcal C_{I}$ that denotes a set of contextual elements in the image $I$ easily detectable by the LVLM. In the extreme case, we can set $\mathcal C_{I}=\emptyset$. \wxy{Use facts and F to replace ground truth, ground truth should be w.r.t a question} Let $\mathcal V_I$ denote the exclusive ground set of all contextual elements in the image $I$. \wxy{I feel we may need a new notation here.} The high-level formulation is then reduced to
\begin{equation}\label{equ:f2s}
    \max_{I,\mathcal C_{Q},\mathcal C_{I}:\mathcal C_{I} \subsetneq \mathcal V_I, \mathcal C_{Q} \cap \mathcal C_{I} =\emptyset} d[f_\mathtt{LVLM}(Q, I), Y_{Q, I}],~~s.t.~~d[f_\mathtt{LLM}(Q, T), f_\mathtt{LVLM}(Q, I)]\leq \epsilon.
\end{equation}
\wxy{check the terms here}

% \wxy{C_I, C_Q}

Note $\mathcal C_{Q}$ is not necessary to be a subset of $\mathcal V_I$ but $\mathcal C_{I}$ should be a subset of $\mathcal V_I$. To avoid information leakage about $\mathcal C_{Q}$ caused by the context elements in $\mathcal C_{I}$, we require $\mathcal C_{Q} \cap \mathcal C_{I}=\emptyset$. 

It is hard to optimize $I$, $\mathcal C_{Q}$, and $\mathcal C_{I}$ by directly solving the problem in Eq.~\ref{equ:f2s}. Hence, in our pipeline, we first probe the LLM prior in LVLM to determine $(\mathcal C_{Q}, \mathcal C_{I})$ such that the elements in $\mathcal C_{Q}$ are highly likely or unlikely present with $\mathcal C_{I}$ in the same scene. This ensures that the language prior is strong and highly confident on the co-occurrence of $(\mathcal C_{Q}, \mathcal C_{I})$, i.e., $\Pr(\mathcal C_{Q} \g \mathcal C_{I})\leq \delta$ ($\mathcal C_{Q}$ is abnormal given $\mathcal C_{I}$) or $\Pr(\mathcal C_{Q} \g \mathcal C_{I})\geq 1-\delta$ ($\mathcal C_{Q}$ is hypothetical given $\mathcal C_{I}$), where $\delta$ is the confidence level. If we make the assumption on such $(\mathcal C_{Q}, \mathcal C_{I})$ pairs that the LVLM reasoning is dominated by the LLM prior, \textit{i.e.} Eq.~\eqref{equ:f2s} holds true, we can create $I$ to maximize the discrepancy $d[f_\mathtt{LVLM}(Q, I), Y_{Q, I}]$. 

\wxy{see if my comments on delta is correct}

According to $\Pr(\mathcal C_{Q} \g \mathcal C_{I})$ of the LLM prior, we can create the query $Q$ and the ground truth answers $Y_{Q, I}$, to maximize the discrepancy between $f_\mathtt{LVLM}(Q, I)$ and $Y_{Q, I}$. For example, when $\mathcal C_{Q}$ and $\mathcal C_{I}$ have high co-occuerence probability, i.e., $\Pr(\mathcal C_{Q} \g \mathcal C_{I}) \geq 1-\delta$, $Q$ can be used to probe if elements in $\mathcal C_{Q}$ are included in an image without $\mathcal C_{Q}$, i.e., $Y_{Q, I} =\vec{0}$. We then generate an image $I$ to be consistent with the fact given in the ground truth information $Y_{Q, I}$ and the guiding text $T$ using a text-to-image model, i.e., $I\sim f_\mathtt{T2I}(Y_{Q, I}, T)$. 

\textbf{Hallucination Attacks.} We position our hallucination attacks for LVLMs centering around a specific adversarial contextual element $q_{adv}$ retrieved by some policies from $\mathcal C_{Q}$, while we create the queries $Q$ and their ground truth answers $Y_{Q, I}$ around $q_{adv}$ accordingly. The adversarial contextual element retrieval strategies covered in this paper include:

\textbf{1. Abnormal Object Insertion.} We intend to find $q_{adv}$ with the \textbf{maximum summation distance} across all contextual elements in $\mathcal C_{I}$, which is:
\begin{align}
    q_{adv} = \arg\max_{q_{adv} \in \mathcal C_{Q}} \sum_{c_i \in \mathcal C_{I}} d(q_{adv}, c_i)
\end{align}
\begin{align}
    q^* = \arg\max_{q \in \mathcal C_{Q}} \sum_{c \in \mathcal C_{I}} d(f_\mathtt{LLM}(q, T), y_{q,I})
\end{align}
where $c_i$ is the $i$-th element in set $\mathcal C_{I}$ and the distance $d$ is hamming distance.

\textbf{2. Correlated Object Insertion.} We intend to find $q_{adv}$ with the \textbf{minimum element-wise distance} among all contextual elements in $\mathcal C_{I}$, which is:
\begin{align}
    q_{adv} = \arg\min_{q_{adv} \in \mathcal C_{Q}} \min_{c_i \in \mathcal C_{I}} d(q_{adv}, c_i)
\end{align}

\textbf{3. Correlated Object Erasure.} We intend to find $q_{adv}$ with the \textbf{minimum summation distance} across all contextual elements in $\mathcal C_{I}$, which is:
\begin{align}
    q_{adv} = \arg\min_{q_{adv} \in \mathcal C_{Q}} \sum_{c_i \in \mathcal C_{I}} d(q_{adv}, c_i)
\end{align}

\wxy{Below this is previous formulation made by Tianyi}

\textbf{High-level Formulation.}
\dianqi{I don't think we need to diff "high-level formulation" and "more specified formulation". We should just jump into the problem we want to explain, and reduce unnecessary notations or descriptions} The goal is to find or generate text-image pairs $(T,I)$ \dianqi{image-text pairs $(I, T)$ ?} such that the LVLM response/answer is dominated by its language model (LM) prior (when LM is exposed to partial information of $I$ in a text form denoted by $T_I$ \dianqi{can't understand this}) but contradicts with the ground truth $y_I$ \dianqi{what's the groundtruth? how to define it?} in the image $I$. Hence, we can formulate the high-level objective as maximizing the distance between the LVLM output probability $\Pr(Y \g T, I)$ \dianqi{What's $Y$? What does $P_r$ mean? why we want to maximize the distance? why maximize the distance is related to our goal?} and the image ground truth $y_I$ \dianqi{This is problematic, $P_r$ is a probability, what's $y_I$? If it's not a probability, then you can't use $d$ to measure the distance.}, while keeping the distance between $\Pr(Y \g T, I)$ and the language model output probability $\Pr(Y \g T, T_I)$ small \dianqi{What's $\epsilon$？}.
\begin{equation}\label{equ:f1}
    \max_{T,I} d[\Pr(Y \g T, I), y_I],~~s.t.~~d[\Pr(Y \g T, T_I), \Pr(Y \g T, I)]\leq \epsilon.
\end{equation}
Another way to explain the above formulation is \dianqi{$LVLM, LM$ are what? are they all functions? what's their relations? }
\begin{equation}
    \max_{T,I} d[\mathtt{LVLM}(T, I), y_I],~~s.t.~~d[\mathtt{LM}(T, T_I), \mathtt{LVLM}(T, I)]\leq \epsilon.
\end{equation}

\textbf{More Specified Formulation.}
\dianqi{define $Q, C, [], V_I, y_Q, y_C$}For example, $T$ can be the questions $T_{I[Q]}$ about a set of contextual elements\footnote{Each contextual element can be a scene, an object, an attribute associated with an object, or the relation between/among multiple objects, similar to the visual genome dataset.} $\mathcal Q$ in or not in the image $I$, while $T_I$ can be the indicators (or labels) $y_{I[C]}$ of a set of contextual elements $C$ in the image $I$ easily detectable by the LVLM. In the extreme case, we can set $\mathcal C=\emptyset$. Let $\mathcal V_I$ denote the set of the ground truths about all contextual elements in the image $I$. The high-level formulation is then reduced to
\begin{equation}\label{equ:f2}
    \max_{I,Q,C:C\subsetneq V_I, Q\cap C=\emptyset} d[\mathtt{LVLM}(T_{I[Q]}, I), y_{I[Q]}],~~s.t.~~d[\mathtt{LM}(T_{I[Q]}, y_{I[C]}), \mathtt{LVLM}(T_{I[Q]}, I)]\leq \epsilon.
\end{equation}
When the questions $T_{I[Q]}$ are all yes/no questions, both the LVLM answer $\mathtt{LVLM}(T_{I[Q]}, I)$ and the ground truth answer $y_{I[Q]}$ can be parsed to binary strings. Hence, we can use Hamming distance as $d[\cdot,\cdot]$ \dianqi{$d$ should be defined in the previous section}. Note $Q$ is not necessary to be a subset of $V_I$ but $C$ should be a subset of $V_I$. To avoid information leakage about $I[Q]$ caused by the context elements in $I[C]$, we require $Q\cap C=\emptyset$. 
With simplified notations, Eq.~\eqref{equ:f2} can be written as
\begin{equation}\label{equ:f2s}
    \max_{I,Q,C:C\subsetneq V_I, Q\cap C=\emptyset} d[\mathtt{LVLM}(T_{Q}, I), y_{Q}],~~s.t.~~d[\mathtt{LM}(T_{Q}, y_{C}), \mathtt{LVLM}(T_{Q}, I)]\leq \epsilon.
\end{equation}

\begin{equation}
    \max_{I,Q,C:C\subsetneq V, Q\cap C=\emptyset} d[f_\mathtt{LVLM}(I, \mathcal{T}({Q})), y_{Q}],~~s.t.~~d[f_\mathtt{LM}(\mathcal{T}({C}), \mathcal{T}({Q})), f_\mathtt{LVLM}(I, \mathcal{T}({Q}))]\leq \epsilon.
\end{equation}
\dianqi{new form, which corresponds to equation (2). While transformation $\mathcal{T}$ transforms the contextual elements in $Q$ into queries, e.g., xxx, it transforms the contextual elements in $C$ into partial fact descriptions in the image, e.g., xxx.}

It is hard to optimize $I$, $Q$, and $C$ by directly solving the problem in Eq.~\ref{equ:f2s}. Hence, in our pipeline, we first probe the LM prior in LVLM to determine $(Q,C)$ such that the elements in $Q$ are highly likely or unlikely present with $C$ in the same scene. This ensures that the language prior is strong and highly confident on the co-occurrence of $(Q,C)$, i.e., $\Pr(Q|C)\leq \epsilon$ ($Q$ is abnormal given $C$) or $\Pr(Q|C)\geq 1-\epsilon$ ($Q$ is hypothetical given $C$). If we make the assumption on such $(Q,C)$ pairs that the LVLM reasoning is dominated by the LM prior, i.e., Eq.~\eqref{equ:f2s} holds true, we can create $I$ to maximize the discrepancy $d[\mathtt{LVLM}(T_{Q}, I), y_{Q}]$. 

According to $\Pr(Q|C)$ of the LM prior, we can create the questions $T_Q$ and their ground truth answers $y_Q$, to maximize the discrepancy between $\mathtt{LVLM}(T_{Q}, I)$ and $y_Q$. For example, when $Q$ and $C$ have high co-occuerence probability, i.e., $\Pr(Q|C)\geq 1-\epsilon$, $T_{Q}$ can ask if elements in $Q$ are included in an image without $Q$, i.e., $y_Q=\vec{0}$ \dianqi{what's $\vec{x}$?}. We then generate an image $I$ to be consistent with the ground truths $y_Q$ and $y_C$ using a text-to-image model, i.e., $I\sim \mathtt{T2I}([y_Q,y_C])$. 

\textbf{Hallucination Attacks.} We position our hallucination attacks for LVLMs centering around a specific adversarial contextual element $q_{adv}$ retrieved by some policies from $Q$, while we create the questions $T_Q$ and their ground truth answers $y_Q$ around $q_{adv}$ accordingly. The adversarial contextual element retrieval strategies covered in this paper include:

\textbf{1. Abnormal Object Insertion.} We intend to find $q_{adv}$ with the \textbf{maximum summation distance} across all contextual elements in $C$, which is:
\begin{align}
    q_{adv} = \arg\max_{q_{adv} \in Q} \sum_i d(q_{adv}, c_i)
\end{align}
where $c_i$ is the $i$-th element in set $C$ and the distance $d$ is hamming distance.

\textbf{2. Correlated Object Insertion.} We intend to find $q_{adv}$ with the \textbf{minimum element-wise distance} among all contextual elements in $C$, which is:
\begin{align}
    q_{adv} = \arg\min_{q_{adv} \in Q} \min_{c_i \in C} d(q_{adv}, c_i)
\end{align}

\textbf{3. Correlated Object Erasure.} We intend to find $q_{adv}$ with the \textbf{minimum summation distance} across all contextual elements in $C$, which is:
\begin{align}
    q_{adv} = \arg\min_{q_{adv} \in Q} \sum_i d(q_{adv}, c_i)
\end{align}

==> section/3_-_problem_formulation_-_old_-_06062024.tex <==
\textbf{Definition and Objectives.} We position our objective to find image-text pairs $(I, T_Q)$ such that the LVLM response $f_\mathtt{LVLM}(I, T_Q)$ is dominant by the same response of its LLM component, $f_\mathtt{LLM}(T_C, T_Q)$, when given a partial fact description $T_C$ about the image $I$ and the same query $T_Q$. In this case, $f_\mathtt{LVLM}(I, T_Q)$ ignores other information presented in the image including the ground truth description $y_{Q}$ with respect to the query.

% prior information of its LLM component $f_\mathtt{LLM}(T_C, T_Q)$ only that could be stimulated by the query $T_Q$ and the guiding text $T_C$ based on a subset of all context elements within the image $I$, and ignore the ground truth information $y_{Q}$ presented in the image $I$ when queried by $T_Q$. 

% given the image $I$ and the probing text $T$ 

% such that the LVLM response/answer is dominated by its language model (LM) prior $Y_{LM}$, generated when LM is exposed to partial information of $I$ (\textit{i.e.} contextual information about a specific part within the image) in a text form denoted by $T_I$ \dianqi{$T$ represents partial description in image $I$}, but contradicts the ground truth $y_I$ \dianqi{$Y_{I, Q}$} in the given image $I$. \wxy{Check if my understanding to LM is correct}

\textbf{A Case Study.} We have an image $I$ depicting an office. This image $I$ has a coffee maker but no perceivable coffee beans inside. The query $T_Q$ is the question to probe the existence of the context \textit{coffee beans} this image, which is \textit{''Is there any coffee beans in this image?''}. The ground truth information $y_{Q}$ in this image $I$ when queried by $T_Q$ is \textit{''There a coffee maker but no coffee beans in this image.''}.
The guiding text $T_C$ extracted from $I$ is usually a \textbf{partial} fact: \textit{''There is a coffee maker in this image.''} In the hallucination case, the LLM prior $f_\mathtt{LLM}(T_C, T_Q)$ under this hallucination case might be \textit{''Yes, there are some coffee beans in this image.''} when exposed to the guiding text $T_C$ and the query $T_Q$. The LVLM output $f_\mathtt{LVLM}(I, T_Q)$, as it is dominated by its LLM prior $f_\mathtt{LLM}(T_C, T_Q)$, might produce a similar answer \textit{''Yes, coffee beans could be found in this image.''}. However, $f_\mathtt{LVLM}(I, T_Q)$ contracts to the ground truth information $y_{Q}$, so hallucination happens.

\wxy{I feel that we need an example from the dataset or PS to illustrate this case}

\textbf{Problem Formulation.} To rigorously formulate this problem, we introduce the idea of contextual distance $d$. When two contexts convey similar information or affirm each other, we denote the contextual distance $d$ between the two is small. On the other hand, if two contexts convey rather irrelevant information or contradict each other, we denote the contextual distance $d$ between the two is large.

Hence, we can formulate the high-level objective function given by  Eq.~\ref{equ:high-level} as maximizing the contextual distance between the LVLM output $f_\mathtt{LVLM}(I, T_Q)$ and the corresponding ground truth information $y_{Q}$, while keeping the contextual distance between $f_\mathtt{LVLM}(I, T_Q)$ and its LLM prior $f_\mathtt{LLM}(T_C, T_Q)$ small enough that the distance between the two is constrained within the upper bound $\epsilon$ denoting the tolerance of the similarity between two contexts. Notably, $T_C$ could be an empty text when the LLM prior is strong enough to cause hallucination in this case.
\begin{equation}\label{equ:high-level}
    \begin{array}{rl}
        \max\limits_{I, T_Q} &d[f_\mathtt{LVLM}(I, T_Q),  y_{Q}], \\
        s.t.&d[f_\mathtt{LVLM}(I, T_Q), f_\mathtt{LLM}(T_C, T_Q) ]\leq \epsilon.
    \end{array}
\end{equation}

\textbf{Set Representation of Contextual Elements.} Semantically, both query $T_Q$ and image $I$ provided to the LVLM could be taken as a combination of several contextual elements\footnote{Each contextual element can be a scene, an object, an attribute associated with an object, or the relation between/among multiple objects, similar to the visual genome dataset.}. Using such a set representation of contextual elements, we could reduce the high-level objective function into a more detailed, set-based objective function focusing on the contextual element conveyed by either query $T_Q$ or image $I$. 

For example, $T_Q$ can be reduced into the query context set $\mathcal Q$ denoting contextual elements in $T_Q$, which could be either in or not in the image $I$. We use $\mathcal{T}(\cdot)$ to denote the mapping between the contextual elements set $\mathcal Q$ and the query text $T_Q$, \textit{i.e.} $T_Q = \mathcal{T}(\mathcal Q)$. $y_{Q}$ is the ground truth information queried from the image $I$ by the query $T_Q$ focusing on the query context set $\mathcal Q$. When the questions $\mathcal{T}(\mathcal Q)$ are all yes/no questions, both the LVLM answer $f_\mathtt{LVLM}(I, \mathcal{T}(\mathcal Q))$ and the ground truth answer $y_{Q}$ can be parsed to binary strings, \textit{i.e.} $0$ denotes counterfactual answers and $1$ denotes the affirmative answers. Hence, we can use Hamming distance as $d[\cdot,\cdot]$ to compute the contextual distance between two contexts. $T_C$ can be the indicators (or labels) $\mathcal C$ that denotes a set of contextual elements in the image $I$ easily detectable by the LVLM. Similarly, we have $T_C = \mathcal{T}(\mathcal C)$. In the extreme case, we can set $\mathcal C=\emptyset$. Let $\mathcal V$ denote the exclusive ground set of all contextual elements in the image $I$. The high-level formulation is then reduced to
\begin{equation}\label{equ:f2s}
\begin{array}{rl}
    \max\limits_{I,\mathcal Q,\mathcal C} &d[f_\mathtt{LVLM}(I, \mathcal{T}({\mathcal Q})), y_{Q}]\\s.t.&d[f_\mathtt{LVLM}(I, \mathcal{T}({\mathcal Q})), f_\mathtt{LLM}(\mathcal{T}({\mathcal C}), \mathcal{T}({\mathcal Q}))]\leq \epsilon,\\
    &\mathcal C\subsetneq \mathcal V, \mathcal Q\cap \mathcal C=\emptyset.
\end{array}
\end{equation}

Note $\mathcal Q$ is not necessary to be a subset of $\mathcal V$ but $\mathcal C$ should be a subset of $\mathcal V$. To avoid information leakage about $\mathcal Q$ caused by the context elements in $\mathcal C$, we require $\mathcal Q \cap \mathcal C=\emptyset$. \tian{Leave some space to probe the bias, otherwise it's hard for the model to say otherwise. }

It is hard to optimize $I$, $\mathcal Q$, and $\mathcal C$ by directly solving the problem in Eq.~\ref{equ:f2s}. Hence, in our pipeline, we first probe the LLM prior in LVLM to determine $(\mathcal Q, \mathcal C)$ such that the elements in $\mathcal Q$ are highly likely or unlikely present with $\mathcal C$ in the same scene. This ensures that the language prior is strong and highly confident on the co-occurrence of $(\mathcal Q, \mathcal C)$, i.e., $\Pr(\mathcal Q \g \mathcal C)\leq \delta$ ($\mathcal Q$ is abnormal given $\mathcal C$) or $\Pr(\mathcal Q \g \mathcal C)\geq 1-\delta$ ($\mathcal Q$ is hypothetical given $\mathcal C$), where $\delta$ is the confidence level. If we make the assumption on such $(\mathcal Q, \mathcal C)$ pairs that the LVLM reasoning is dominated by the LLM prior, \textit{i.e.} Eq.~\eqref{equ:f2s} holds true, we can create $I$ to maximize the discrepancy $d[f_\mathtt{LVLM}(I, \mathcal{T}({\mathcal Q})), y_{Q}]$. 

\wxy{see if my comments on delta is correct}

According to $\Pr(\mathcal Q \g \mathcal C)$ of the LLM prior, we can create the query $T_Q$ and the ground truth answers $y_{Q}$, to maximize the discrepancy between $f_\mathtt{LVLM}(I, \mathcal Q)$ and $y_{Q}$. For example, when $\mathcal Q$ and $\mathcal C$ have high co-occuerence probability, i.e., $\Pr(\mathcal Q \g \mathcal C) \geq 1-\delta$, $T_Q$ can be used to probe if elements in $\mathcal Q$ are included in an image without $\mathcal Q$, i.e., $y_{Q} =\vec{0}$. We then generate an image $I$ to be consistent with the fact given in the ground truth information $y_{Q}$ and the guiding text $\mathcal{T}({\mathcal C})$ using a text-to-image model, i.e., $I\sim f_\mathtt{T2I}(y_{Q}, \mathcal{T}({\mathcal C}))$. 

\textbf{Hallucination Attacks.} We position our hallucination attacks for LVLMs centering around a specific adversarial contextual element $q^*$ retrieved by some policies from $\mathcal Q$, while we create the queries $T_Q$ and their ground truth answers $y_{Q}$ around $q^*$ accordingly. The adversarial contextual element retrieval strategies covered in this paper include:

\textbf{1. Abnormal Object Insertion.} We intend to find $q^*$ with the \textbf{maximum summation distance} between its language prior and the ground truth information across all contextual elements in $\mathcal C$, which is:
\begin{align}
    q^* = \arg\max_{q \in \mathcal Q} \sum_{c \in \mathcal C} d(f_\mathtt{LLM}(\mathcal{T}(c), \mathcal{T}(q)), y_{q})
\end{align}
where $q$ is one element in the query context set $\mathcal Q$ and $c$ is one element in the image context set $\mathcal C$. The distance $d$ is the hamming distance. $\mathcal{T}(q)$ and $\mathcal{T}(c)$ are corresponding context for $q$ and $c$. $y_{q}$ is the ground truth information regarding the contextual element $q$.

\textbf{2. Correlated Object Insertion.} We intend to find $q^*$ with the \textbf{minimum element-wise distance} between its language prior and the ground truth information among all contextual elements in $\mathcal C$, which is:
\begin{align}
    q^* = \arg\min_{q \in \mathcal Q} \min_{c \in \mathcal C} d(f_\mathtt{LLM}(\mathcal{T}(c), \mathcal{T}(q)), y_{q})
\end{align}

\textbf{3. Correlated Object Erasure.} We intend to find $q^*$ with the \textbf{minimum summation distance} between its language prior and the ground truth information across all contextual elements in $\mathcal C$, which is:
\begin{align}
    q^* = \arg\min_{q \in \mathcal Q} \sum_{c \in \mathcal C} d(f_\mathtt{LLM}(\mathcal{T}(c), \mathcal{T}(q)), y_{q})
\end{align}


==> section/4_-_method_-_old_-_06072024.tex <==
\section{Methodology}


% We assume that for a given scene image, its contextual information contributes to its determinative definition over other candidates and comes from the composition of the contextual elements within the scene background and other existing indicative objects.
%
% On the basis of our analysis of the contextual cues that cause hallucination, 
Based on our problem formulation and inspired by concepts from cognitive science, we propose two primary strategies to induce hallucination due to strong language and contextual priors: inserting abnormal objects and removing objects that are strongly correlated with the context.
% . One of them is to insert abnormal objects versus existing objects and scene backgrounds. Such insertion objects must convey clear information irrelevant to the context presented by existing objects and the scene background. The other is to erase the hypothetical objects that have strong implicate with one or more perceivable objects or backgrounds within the image. Such objects should be presented in the given scene by default with the existence of other correlated contextual elements but be erased intentionally.
%
The overall pipeline is presented in Fig. XX. \wxy{Insert overview images and captions here.}

For each strategy, we first give an overview of the approach with an example. After that, we break down the automated process into 4 stages: scene generation, manipulation of the target object, question construction and hallucination detection.

% \jbgcomment{I think there needs to be a clearer transition from the previous section: e.g., now that we have $\mathcal{W}$, we \dots }


% \subsection{Context Creation and Probing}



% \subsection{Scene Generation}

% \subsubsection{Context Image Generation}

% \subsubsection{Object Generation and Insertion}

% \subsubsection{Object Removal}




% \subsection{Abnormal Object Hallucination}
% \subsection{Hallucination under Strong Context}

\subsection{Hallucination about Abnormal Object Insertion into Strong Context}
\label{Methodology: Abnormal Object given Strong Context}

Hallucinations caused by abnormal object insertion usually happen when the added object contradicts with the strong contextual information in the given image. 
% We assume that the existing contextual elements, including the indicative objects and background, are contextually correlated with each other and construct a strong language prior. 
% To construct the hallucination case, the inserted objects perturb abnormal contextual information negatively correlated with the current language prior. 
For example, when we provide an image of an office, with a desk, a computer, and a chair presented, the adversary object that contradicts with this context could be a cooking pot. 
% The internal conflicts within the existing solidated language prior to and the perturbed abnormal adversary objects could contribute to the failure to identify the existence or spatial relations of the perturbed abnormal objects or make consistent, reasonable answers throughout the evaluation question series.

\wxy{Insert some pointers to the showcases here.}

\subsubsection{Scene Creation}

In the abnormal object insertion strategy, we first use the LVLM to incur a scene name, which could be done with or without extra constraints over the incurring scope. With the given scene name, we use the target LVLM to retrieve several contextual elements to enhance language prior given by the scene, where in this case, these objects are several most relevant objects given the scene. With the scene name and several correlated objects given the scene context, we use the diffusion model or image generative model like DALL-E 3~\cite{dalle3} to generate the image with strong language prior that contains the retrieved scene information and relevant objects.

\subsubsection{Insertion of Abnormal Object}

After we obtain the scene image with those generated context, we probe and ask the victim LVLMs to generate a abnormal object that is negatively correlated with existing contextual elements with in scene image. We use DALL-E 3~\cite{dalle3} to create this image, or choose from an existing database of images.

To guarantee the insertion is successful and does not introduce any artifacts, we simply stitch the object into the scene image after removing the background of the object image~\cite{backgroundremover2021} instead of using diffusion or in-painting method.


% Given the strong contextual prior within the image to attack, we use the victim LVLM to retrieve one object negatively correlated with existing contextual elements. We use the DALL-E 3~\cite{dalle3} to create an image solely containing the object for insertion. In our current pipeline, we use a vanilla object stitch method that removes the background of the object image \wxy{cite this: https://github.com/nadermx/backgroundremover} and stitch the object figure with a transparent background into a random place within the image for manipulation. Our experiment results reveal the efficiency of these primitive methods, though it still leaves space for further improvement of object stitching and inpainting methods. 



% Apart from our current irrelevant object retrieval design, we conduct ablation studies to discuss the performance of the adversarial attacks over the size of the perturbed objects and the object choices over their relevance to the existing language priors in the experimentation section \wxy{Replace with pointer later}. We also present some ablation studies that constrain the scope of object retrieval when manipulation and analyze the effect under such experiment settings.

\subsubsection{Question Construction}
\label{Methodology: Question Construction}
We mainly ask two types of questions: existence of the added object and spatial relation between this object and other objects in the scene.

In existence questions, we directly ask whether the inserted object is present in the image. These questions are repeated multiple times, incorporating varying levels of detail and supplementary information as part of the prompt and query. For example, we ask the same victim model to generate image caption and add this text in front of the query question, as such supplementary information may serve as another source of language prior that misleads the victim model. 
In addition, we also ask existence questions on objects that are missing in the image caption generated by the victim model because it has higher probability to miss this object again in the existence question.

% when different levels of supplementary information are provided to the victim model as we ask the same existence question both with and without the image captioning generated by the same victim model, as such supplementary information may serve as another source of language prior that misleads the victim model. 

% We also question the existence of those existing scene objects that are detectable by the object detection model but missing in the image captions generated by the victim model.

% We propose two major textual probing methods for potential hallucinations. One of them is to ask existence questions about the inserted abnormal objects that we directly ask whether the perturbed objects exist in the given image. Such existence questions are repeated when different levels of supplementary information are provided to the victim model as we ask the same existence question both with and without the image captioning generated by the same victim model, as such supplementary information may serve as another source of language prior that misleads the victim model. We also question the existence of those existing scene objects that are detectable by the object detection model but missing in the image captions generated by the victim model.

In spatial relation question, we ask about the relative position between the abnormal object and the detected scene objects. We use heuristic policy to determine the spatial relations between the perturbed object and the detected scene objects by comparing their center positions. The spatial relations are divided into $5$ categories: \textit{Left}, \textit{Right}, \textit{Above}, \textit{Below}, \textit{Front} (when the perturbed object overlaps with the scene object). Spatial relation questions are asked both with and without object-level description generated by the victim model. 

% Another textual probing perspective is to question the spatial relations between the perturbed abnormal object and the detected scene objects. We use heuristic policy to determine the spatial relations between the perturbed object and the detected scene objects by comparing their center positions. The spatial relations are divided into $5$ categories: \textit{Left}, \textit{Right}, \textit{Above}, \textit{Below}, \textit{Front} (when the perturbed object overlaps with the scene object). Spatial relation questions are asked both with and without descriptive information generated by the victim model for the scene object provided in the question. 

\subsubsection{Hallucination Detection}

We use GPT4-V~\cite{2023GPT4VisionSC} to evaluate the correctness of the predicted answer by the victim model and the ground truth. There are two criteria to determine whether hallucination occurs with different levels of reliability:

\begin{enumerate*}
    \item \textbf{Correctness:} Since we know the ground truth existence and relations of objects, we can easily determine the correctness of the visual question pairs. This criterion is the most straight-forward, but it does not account for any generation errors or background-removal artifacts from the pipeline. If some of the steps fail, the ground truth may not be reliable. 
    % happens when the victim LVLM fails to detect perturbed objects that actually exist from the given image or makes mistakes in determining the spatial relations between perturbed objects and scene objects.
    % In this case, we assume that there are no error in between.
    \item \textbf{Inconsistency:} In this criterion, we want to consider the consistency of the model outputs, which does not rely on whether the ground truth is accurate. For example, if we ask the existence of an object and get different responses, we are certain that one of the response is hallucinating. 
\end{enumerate*}

% as the judgment model that reads the question, the prediction answer made by the victim model, and the reference information generated when preparing the case which could either the ground truth produced heuristically or the supplementary information generated by the victim model. Potential hallucinations probed with questions asked by our approach could be divided into the following cases: 

% \jbgcomment{I'm assuming that this is with respect to object sets.  How do you test membership in those sets to make these decisions?  What about equivalent non-string identical mentions?  (E.g., "ball" vs. "sphere").}

% \begin{enumerate*}
%     \item \textbf{Direct Hallucination (for Perturbation)} happens when the victim LVLM fails to detect perturbed objects that actually exist from the given image or makes mistakes in determining the spatial relations between perturbed objects and scene objects.
%     \item \textbf{Answer Inconsistency (for Perturbation)} happens when the victim LVLM fails to make consistent answers (which could be either all correct or all wrong) to the existence of the perturbed object or the spatial relations when varying contextual information produced by this victim model provided.
%     \item \textbf{Local-Global Inconsistency (for Perturbation)} happens when the victim model fails to provide consistent answers when generating captions to the vanilla pre-manipulation object figure and making predictions given the post-manipulation images.
% \end{enumerate*}

% \subsection{Hypothetical Object Hallucination}
% \subsection{Erasure of Hypothetical Object}
% \subsection{Removal of Strong Correlation}
% \subsection{Hallucination under Strong Correlation}

\subsection{Hallucination about Correlated Object Absence from Strong Context}
\label{Methodology: Object given Correlated Objects}

Hallucinations raised from the absence of correlated objects given a strong context always happen when one or multiple objects correlated with the absent object exist in the image. This strong correlation suggests a usual co-occurrence between the perceivable context and the absent objects.
%
% Hallucinations caused by the absence of hypothetical objects always happen when one indicative objects with strong positive contextual correlation with existing contextual elements, which could be either objects or backgrounds. Such strong prior always implies the co-occurrence of the perceivable contextual elements and the absent hypothetical objects, which lays the foundation of the hallucination cases we intend to construct via this strategy.
%
This strategy is split into two approaches. The first involves selecting two correlated objects, like a coffee machine and coffee beans. We introduce one object, like the coffee machine, into a target image, omitting the other. The hallucinated LVLM asserts the existence of hypothetical coffee beans, given the existence of the coffee machine.
% This strategy could be divided into two sub-categories: one of them is to find two co-occurrence objects, \textit{e.g.} coffee machine and coffee beans, insert one object into the victim image, and leave the other absent. Apart from the textual probing pipeline we use in the abnormal object insertion strategy, we probe the vulnerability of LVLM to such correlated objects by questioning the existence of the invisible correlated objects with varying levels of contextual information.
% 
The second approach involves deliberately removing an object from a scene having multiple correlated objects within, such as erasing a computer from an office image but keeping the desk and chairs. We explore hallucinations by querying the existence and spatial relationships of the removed objects and identify inconsistencies in responses to these queries.
% The other sub-strategy is to intentionally erase one indicative object from one scene image with complete contextual information. For example, we will erase and refill the computer region with something else, and preserve other contextual elements, like desks and chairs, within the office image as the victim. We probe the hallucinations by asking existence and spatial relation questions about the hypothetical objects and detect the inconsistency among answers to different questions with the same targets.

\wxy{Insert some pointers to the showcases here.}

\subsubsection{Scene Creation}

In the correlated object absence approach, we use two pipelines for our sub-strategies. For the sub-strategy involving hypothetical objects correlated with only one object within the image, our process mirrors the abnormal object insertion: using LVLM to query scenes with potential constraints to enhance language priors through correlated object retrieval.
%
%In the hypothetical object erasure strategy, we conduct two scene creation pipelines to tackle the difference between both sub-strategies. For the sub-strategy that the hypothetical objects correlated with the perturbed objects within the manipulated image, we follow a very similar pipeline as we did in the abnormal object insertion that we use LVLM to randomly query the scene with or without some pre-defined constraints and retrieve several correlated objects to enhance the language prior.

In the sub-strategy where we erase an indicative object from an image, we employ LVLM to simply retrieve a scene name. Using a generative image model, such as DALL-E 3~\cite{dalle3}, we then produce an image rich in contextual elements without imposing additional constraints on the objects present, expecting the image to naturally include objects highly correlated with the specified scene.
%
% For the sub-strategy that erases the existing indicative object from the existing image, we only use the LVLM to randomly retrieve a scene name and use the generative image model~\cite{dalle3} to produce an image with sufficient contextual elements. We do not apply any extra constraints over the objects mandatory contained within this image so we assume the outcome image should contain those objects with the strongest correlation with the given scene.

\subsubsection{Absence of Correlated Object}

To achieve the absence of the object correlated with the existing contextual elements, we propose different contextual information erasure methods accordingly for each sub-strategy. In the case that one absent object correlated with another perturbed object, we use the generative image model~\cite{dalle3} to generate the idle object image with the necessary inspection mechanism to ensure the tidiness of the contextual cues in the image generated. After removing the background, the idle object figure with a strong correlation with the absent hypothetical objects is stitched in the manipulated image to create hallucination cases. 

For the sub-strategy that erases the existing indicative object with a strong correlation with multiple contextual elements in the target image having the strong language prior, we first use the victim LVLM to detect all contextual elements within the given scene image, then use the object detection model \cite{minderer2022simple} to detect and segment all candidate contextual elements for erasure from the image. We randomly pick one contextual element to erase. We use the generative image model DALL-E-2 \cite{ramesh2022hierarchical} to inpaint the region of the chosen object for erasure with something else. We utilize some insurance mechanism that keeps detecting and erasing all potential contextual elements to avoid any further interference with the later evaluation logic.


\subsubsection{Question Construction}
For the sub-strategy that the absent object is correlated with one perturbed object, we introduce the extra series of questions that probe the existence of the hypothetical object apart from the normal textual probing procedure for the abnormal object insertion strategy. We probe the hallucinations by asking existence questions with three levels of contextual information provided, including the vanilla existence question, the existence question with descriptive information for the perturbed object generated by the victim model, and the existence question with the detailed caption for the whole image.

When the absent object has a strong correlation with multiple contextual elements within the image, the focus of the textual probing switches to the existence and spatial relations with the hypothetical object since its strong correlation with the existing contextual element implies its existence, which paves the way towards the hallucination constructions. The modified existence probing for the hypothetical object includes existence questions complied by four levels of contextual information: vanilla (no extra information), descriptive information of the hypothetical object that is generated by the victim LVLM before erasure, concatenated descriptive information of the perceived objects correlated with the hypothetical object, detailed captions for the whole image. The modified spatial relation questions targeting the hypothetical object include spatial relation questions both with and without the descriptive information of the hypothetical object provided. The spatial relations between the hypothetical object and the remaining objects are generated heuristically using the bounding box of the hypothetical object before removal and those bounding boxes of detected contextual elements after image manipulation.

\subsubsection{Hallucination Detection}

The hallucination detection mechanism for those caused by the absence of correlated objects follows the same structure proposed in the other strategy that uses GPT-4v to evaluate the correspondence between the model prediction and the reference text. Apart from those hallucination cases detectable by the existence and spatial relation textual probe, the absence of correlated object strategy with both one perturbed object and multiple existing contextual elements induces the following extra hallucination cases identically introduced by the absent objects with strong contextual correlations: 

\begin{enumerate}
    \item \textbf{Correctness} happens when the victim LVLM mistakenly assumes the existence of a hypothetical object that is actually absent from the given image or makes wrong assumptions in determining the spatial relations between hypothetical objects and any scene objects, \textit{i.e.} try to make decisive prediction over spatial relations for some absent objects.
    \item \textbf{Inconsistency} happens when the victim LVLM fails to make consistent answers (which could be either all correct or all wrong) to the existence of the hypothetical object or the spatial relations when varying contextual information produced by this victim model is provided.
\end{enumerate}




% \subsection{Textual Probing}

==> section/6-exp.tex <==
\section{Experiments}

\jbgcomment{Remember that the reviewers are not required to read the appendix.  I realize that space is thight, but I think at least one image needs to be in the main body text.  You can encourage the reviewers to look at more images by discussing qualitative examples in the text.  I'd suggest one of the following:

\begin{itemize}
    \item Issues with the image editing, i.e., where a human would not understand that an object was added
    \item Example where all models successfully "see" the edit
    \item Example where all models don't "see" the edit
    \item Example where the straightforward evaluation doesn't work (e.g., because of answer equivalence issues)
\end{itemize}

Even if you can't fit the images in, discussing them and forwardpointing to the appendix will ensure that reviewers actually look at them.  
}

\subsection{Experiment Design}
We conduct several experiments to evaluate the performance of three hallucination attack strategies, \textbf{Abnormal Object Insertion}, \textbf{Correlated Object Insertion}, and \textbf{Correlated Object Erasure}, over different victim models, including closed-source LVLMs like GPT4-V-Turbo \cite{yang2023dawn}, Gemini \cite{google_gemini}, Claude \cite{claude3}, and open-source LVLMs like Llava \cite{liu2023improved}, and miniGPT4 \cite{zhu2023minigpt}. We perform experiments over self-generated datasets in which images and objects are retrieved by language models and generated by generative image models, and real-world datasets that use scene images and objects segmented from real-world images. Specifically, we use the scene and object dataset sampled from the COCO dataset \cite{lin2014microsoft}.

Along with experiments conducted on different datasets, we also perform several ablation studies over several context query and sample generation strategies, including the effect of the object size to be perturbed into the image, the backbone models retrieving the objects for perturbation, and the strategy that decides which objects for perturbation over its relevance to the existing context elements. We will analyze the phenomena we encounter from experiment results in depth to shed insights into the causes that contribute to the emergence of hallucination from our cases.

\subsection{Results}
\subsubsection{Self-generated Dataset}
Table. \ref{basic_results}

\subsubsection{Aligned Dataset}
Table. \ref{reuse_results}

\subsubsection{Real-world Dataset}
Table. \ref{real_results}

\subsection{Ablation Studies}
\subsubsection{The Effect of Object Sizes}
Table. \ref{ablation_window}

\subsubsection{Probe with Different LVLMs}
(Later)

Table. \ref{ablation_probe}

\subsubsection{The Effect of Relevance for Inserted Objects}
Table. \ref{ablation_random}


\subsection{Discussion}
Across all results, we derive several insights that 

(Find at least 5 points )
\textbf{Inconsistency Contributes to Hallucination.}

\textbf{Robust to Absence, Vulnerable to Perturbation.}

\textbf{Robustness to Hallucination Attacks across LVLMs.}

\textbf{Reality Increases Difficulty.}

\textbf{Larger, Robuster.}

\wxy{Another about Swaped obj retrieval.}

==> tables/ablation_probing.tex <==
\begin{table*}[h]
  \begin{center}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccccccccccc}
    \toprule
        \multicolumn{2}{c}{LVLMs} & \multicolumn{3}{c}{\makecell{Overall}}
        & \multicolumn{3}{c}{\makecell{Existence}} & \multicolumn{3}{c}{\makecell{Spatial Relation}} \\
        \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
        \makecell{Obj. \\ Retrieval} & \makecell{Img. \\ Caption} & \makecell{Overall \\ ASR} & \makecell{Overall \\ MASR} & \makecell{Overall \\ CASR} & \makecell{Exi. \\ ASR} & \makecell{Exi. \\ MASR} & \makecell{Exi. \\ CASR} & \makecell{Sp. \\ ASR} & \makecell{Sp. \\ MASR} & \makecell{Sp. \\ CASR}\\
        \midrule
        GPT4V & Gemini & 96.0 & 87.5 & 89.5 & 84.5 & 66.5 & 73.0 & 83.8 & 65.4 & 75.4\\
        Gemini & GPT4V & 94.0 & 78.5 & 91.5 & 89.5 & 59.5 & 84.5 & 84.8 & 75.6 & 63.4\\
        GPT4V & LlaVA & 95.1 & 86.0 & 89.7 & 87.5 & 66.0 & 85.4 & 85.3 & 67.9 & 75.1\\
        LlaVA & GPT4V & 96.5 & 81.0 &  94.5 & 93.0 & 64.5 & 91.5 & 82.6 & 73.9 & 69.6\\
        Gemini & LlaVA & 96.6 & 87.0 & 91.4 & 86.1 & 67.6 & 74.9 & 85.5 & 72.4 & 67.1\\
        LlaVA & Gemini & 94.5 & 84.0 & 87.0 & 87.0 & 72.5 & 73.5 & 85.5 & 69.0 & 73.7\\
    \hline
    \end{tabular}
    }
    \end{center}
    \caption{\textbf{Ablation Study: Attack Results using different combinations of abnormal object retrieval and image caption models in the abnormal object insertion experiment.} \tian{Can be removed}} 
    \label{ablation_probe}
\end{table*}
